EWareNet: Emotion Aware Human Intent Prediction and Adaptive Spatial Profile Fusion for Social Robot Navigation

We present EWareNet, a novel intent and affect-aware social robot navigation algorithm among pedestrians. Our approach predicts the trajectory-based pedestrian intent from gait sequence, which is then used for intent-guided navigation taking into account social and proxemic constraints. We propose a transformer-based model that works on commodity RGB-D cameras mounted onto a moving robot. Our intent prediction routine is integrated into a mapless navigation scheme and makes no assumptions about the environment of pedestrian motion. Our navigation scheme consists of a novel obstacle profile representation methodology that is dynamically adjusted based on the pedestrian pose, intent, and affect. The navigation scheme is based on a reinforcement learning algorithm that takes pedestrian intent and robot's impact on pedestrian intent into consideration, in addition to the environmental configuration. We outperform current state-of-art algorithms for intent prediction from 3D gaits.

==> misc/notes-bala.tex <==
-----------------
General
-----------------
- uncertainity of sensor space - how is this addressed?
- Transformer networks - literature review
- Training procedure - how transformers are trained - data used for training transformers
how emotion classification network is trained - data used there

- Training plan, rewards definition- example - https://arxiv.org/pdf/2206.10028.pdf

-----------------------
metrics
-----------------------
- cite different metrics
- For pedestrian prediction - average displacement

error and final displacement error - https://intuitivecomputing.jhu.edu/publications/2020-icra-katyal.pdf - this paper takes supervised learning approach to solve the intent prediction proiblem - [24, 23] - datasets
- For Path planning - Cost function - https://www.comp.nus.edu.sg/~leews/publications/bai2015intention.pdf
- For path planning metrics - https://arxiv.org/pdf/1805.11833.pdf

---------------------
Dataset paper 
----------------------
- https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.107.3028&rep=rep1&type=pdf - trajectories with walking sequences - How dataset is built using examples by taking the closely matched scenario - influence functions - problem with our dataset.

---------------------
Training method - cite
---------------------
- procedure?

----------------------
Related Papers
----------------------
- https://arxiv.org/pdf/2206.10028.pdf
